FLAG Review 2024

We review lattice results related to pion, kaon, $D$-meson, $B$-meson, and nucleon physics with the aim of making them easily accessible to the nuclear and particle physics communities. More specifically, we report on the determination of the light-quark masses, the form factor $f_+(0)$ arising in the semileptonic $K \to \pi$ transition at zero momentum transfer, as well as the decay-constant ratio $f_K/f_\pi$ and its consequences for the CKM matrix elements $V_{us}$ and $V_{ud}$. We review the determination of the $B_K$ parameter of neutral kaon mixing as well as the additional four $B$ parameters that arise in theories of physics beyond the Standard Model. For the heavy-quark sector, we provide results for $m_c$ and $m_b$ as well as those for the decay constants, form factors, and mixing parameters of charmed and bottom mesons and baryons. These are the heavy-quark quantities most relevant for the determination of CKM matrix elements and the global CKM unitarity-triangle fit. We review the status of lattice determinations of the strong coupling constant $\alpha_s$. We review the determinations of nucleon charges from the matrix elements of both isovector and flavour-diagonal axial, scalar and tensor local quark bilinears, and momentum fraction, helicity moment and the transversity moment from one-link quark bilinears. We also review determinations of scale-setting quantities. Finally, in this review we have added a new section on the general definition of the low-energy limit of the Standard Model.

==> NME/Tables/app_actions.tex <==
\begin{table}[h]
\mbox{} \\[-0.5cm]
\footnotesize
\begin{tabular*}{\textwidth}[l] {l @{\extracolsep{\fill}} c c c c }\hline\hline\\[-1.0ex]
 Collab. & Ref. & $\Nf$ &  \parbox{1cm}{gauge\\action} &  \parbox{1cm}{quark\\action} \\
&& &&\\[-0.1cm]
\hline
\hline
&& &&\\[-0.1cm]
ETM 15D,16A,17B,17C,17 & \cite{Abdel-Rehim:2015owa,Abdel-Rehim:2016won,Alexandrou:2017hac,Alexandrou:2017oeh,Alexandrou:2017qyt} & 2 & Iwasaki  & tmWil$^{\$}$  \\[0.5ex] 
JLQCD 08B & \cite{Ohki:2008ff} & 2 &  Iwasaki & overlap  \\[0.5ex] 
Mainz 12,17 & \cite{Capitani:2012gj,Capitani:2017qpc} & 2 &  Wilson & npSW  \\[0.5ex] 
QCDSF 06,12,13 & \cite{Khan:2006de,Bali:2012qs,Horsley:2013ayv} & 2 &  Wilson & npSW  \\[0.5ex] 
RBC 08 & \cite{Lin:2008uz} & 2 &  DBW2 & DW  \\[0.5ex] 
RQCD 14,16 & \cite{Bali:2014nma,Bali:2016lvx} & 2 &  Wilson & npSW  \\[0.5ex] 
\hline
$\chi$QCD 13A,15 & \cite{Gong:2013vja,Gong:2015iir} & 2+1 & Iwasaki  & DW$^{\star}$  \\[0.5ex] 
$\chi$QCD 18 & \cite{Liang:2018pis} & 2+1 & Iwasaki  & DW,M-DW$^{\star}$  \\[0.5ex] 
$\chi$QCD 15A & \cite{Yang:2015uis} & 2+1 & Iwasaki  & M-DW$^{\star}$  \\[0.5ex] 
BMW 15 & \cite{Durr:2015dna} & 2+1 &  tlSym & HEX-tlSW  \\[0.5ex] 
BMW 11A & \cite{Durr:2011mp} & 2+1 &  tlSym & stout-tlSW  \\[0.5ex] 
Engelhardt 12 & \cite{Engelhardt:2012gd} & 2+1 & tadSym  & Asqtad$^{\dagger}$  \\[0.5ex] 
JLQCD 12A,18 & \cite{Oksuzian:2012rzb,Yamanaka:2018uud} & 2+1 &  Iwasaki & overlap  \\[0.5ex] 
Junnarkar 13 & \cite{Junnarkar:2013ac} & 2+1 & tadSym  & Asqtad$^{\dagger}$  \\[0.5ex] 
LHPC 05,10 & \cite{Edwards:2005ym,Bratt:2010jn} & 2+1 & tadSym  & Asqtad$^{\dagger}$  \\[0.5ex] 
LHPC 12,12A & \cite{Green:2012ej,Green:2012ud} & 2+1 &  tlSym & HEX-tlSW  \\[0.5ex] 
MILC 09D,12C & \cite{Toussaint:2009pz,Freeman:2012ry} & 2+1 &  tadSym & Asqtad  \\[0.5ex] 
Mainz 18 & \cite{Ottnad:2018fri} & 2+1 &  tlSym & npSW  \\[0.5ex] 
Martin~Camalich 10 & \cite{MartinCamalich:2010fp} & 2+1 &  Iwasaki & npSW  \\[0.5ex] 
PACS 18 & \cite{Ishikawa:2018rew} & 2+1 &  Iwasaki & npSW  \\[0.5ex] 
PACS-CS 09 & \cite{Ishikawa:2009vc} & 2+1 &  Iwasaki & npSW  \\[0.5ex] 
QCDSF 11 & \cite{Horsley:2011wr} & 2+1 &  tlSym & npSW  \\[0.5ex] 
RBC/UKQCD 08B,09B,10D & \cite{Yamazaki:2008py,Yamazaki:2009zq,Aoki:2010xg} & 2+1 &  Iwasaki & DW  \\[0.5ex] 
Shanahan 12 & \cite{Shanahan:2012wh} & 2+1 &  Iwasaki & npSW  \\[0.5ex] 
\hline
CalLat 17,18 & \cite{Berkowitz:2017gql,Chang:2018uxx} & 2+1+1 & tadSym  & HISQ$^{\#}$  \\[0.5ex] 
ETM 14A & \cite{Alexandrou:2014sha} & 2+1+1 & Iwasaki  & tmWil$^{\$}$  \\[0.5ex] 
MILC 12C & \cite{Freeman:2012ry} & 2+1+1 &  tadSym & HISQ  \\[0.5ex] 
PNDME 13,15,16,18B,18A,18 & \cite{Bhattacharya:2013ehc,Bhattacharya:2015wna,Bhattacharya:2015esa,Bhattacharya:2016zcn,Gupta:2018lvp,Lin:2018obj,Gupta:2018qil} & 2+1+1 & tadSym  & HISQ$^{\ddag}$  \\[0.5ex] 
\hline
\hline
\end{tabular*}
\begin{minipage}{\linewidth} 
{\footnotesize 
\begin{itemize} 
 \item[$^{\$}$]  Calculations involving the strange and charm quarks use Osterwalder-Seiler~\cite{Osterwalder:1977pc} fermions for these quark flavours. \\[-5mm]
 \item[$^{\star}$]  The calculation uses overlap fermions in the valence quark sector. \\[-5mm]
 \item[$^{\dagger}$]  The calculation uses DW fermions in the valence quark sector. \\[-5mm]
 \item[$^{\#}$]  The calculation uses M-DW fermions in the valence quark sector. \\[-5mm]
 \item[$^{\ddag}$]  The calculation uses mfSW fermions in the valence quark sector. \\[-5mm]
\end{itemize}
}
\end{minipage}
\caption{Summary of simulated lattice actions for calculations in Sec.~\ref{sec:NME}.
\label{tab:NME lattice actions}}
\end{table}


==> NME/Tables/app_ga_singlet.tex <==
\clearpage
\begin{table}[!ht]
{\footnotesize
\begin{tabular*}{\textwidth}{l @{\extracolsep{\fill}} c c c l}
\hline\hline \\[-1.0ex]
Collab. & Ref. & $\Nf$ & $a$ [fm] & Description 
\\[.3ex]\\[-2.ex] \hline \hline \\[-1.0ex]
%
%%% SS
ETM 19 & \cite{Alexandrou:2019brg} & 2+1+1 & 0.08 & \parbox[t]{6.3cm}{Not estimated. }
\\[0.5ex]\\[0.5ex]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifx\reducedapptables\undefined
\hline \\[-0.5ex]
PNDME 18A & \cite{Lin:2018obj} & 2+1+1 & 0.15,0.12,0.09,0.06 & \parbox[t]{4.7cm}{  Connected: Joint continuum, chiral and volume fit with a term linear in $a$. \\ Disconnected: Joint continuum and chiral fit with a term linear in $a$. }   \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
$\chi$QCD 18 & \cite{Liang:2018pis} & 2+1 & 0.14,0.11,0.08 & \parbox[t]{4.7cm}{Joint continuum and chiral fit with a term linear in $a^2$.}   \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
JLQCD 18 & \cite{Yamanaka:2018uud} & 2+1 & 0.11 &  \parbox[t]{4.7cm}{  Discretization effects are estimated to be $8\%$ using $\cO(\Lambda^2_{QCD}a^2)$ with $\Lambda_{QCD}\approx 500$~MeV.}   \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
$\chi$QCD 15 & \cite{Gong:2015iir} & 2+1 & 0.11 & \parbox[t]{4.7cm}{ Single lattice spacing.}   \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
Engelhardt 12 & \cite{Engelhardt:2012gd} & 2+1 & 0.12 &  \parbox[t]{4.7cm}{ Single lattice spacing.}  \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
ETM 17C & \cite{Alexandrou:2017oeh} & 2 & 0.09 & \parbox[t]{4.7cm}{ Single lattice spacing.}  \\[0.5ex]\\[0.5ex]
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hline \hline \\[-1.0ex]
\end{tabular*}
\caption{
\ifx\reducedapptables\undefined
Continuum extrapolations/estimation of lattice artifacts in
  determinations of $g_A^q$.
\else
Continuum extrapolations/estimation of lattice artifacts in
  determinations of $g_A^q$ and $g_T^q$.
\fi
}
}
\end{table}

\begin{table}[!ht]
{\footnotesize
\begin{tabular*}{\textwidth}{l @{\extracolsep{\fill}} c c c l}
\hline\hline \\[-1.0ex]
{Collab.} & {Ref.} & {$\Nf$} & {$M_{\pi,\rm min}\,[\mev]$} & {Description}  
\\[.3ex]\\[-2.ex] \hline \hline \\[-1.0ex]
%
%%% SS 
ETM 19 & \cite{Alexandrou:2019brg} & 2+1+1 & 139  & \parbox[t]{6.3cm}{ Simulate close to $M_\pi^{phys}$. }
\\[0.5ex]\\[0.5ex]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifx\reducedapptables\undefined
\hline \\[-0.5ex]
PNDME 18A & \cite{Lin:2018obj} & 2+1+1 &  \parbox[t]{2.5cm}{ $C$: 320,225,135 \\ $D_l$: 320, 235 \\ $D_s$: 320, 225, 138} &  \parbox[t]{4.7cm}{  Connected: Joint continuum, chiral and volume fit with a term linear in $M_\pi^2$. \par Disconnected: Joint continuum and chiral fit with a term linear in $M_\pi^2$. }  \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
$\chi$QCD 18 & \cite{Liang:2018pis} & 2+1 & 171,337,302 & \parbox[t]{4.7cm}{Joint continuum and chiral fit with a term linear in $M_{\pi,{\rm val}}^2$.}   \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
JLQCD 18 & \cite{Yamanaka:2018uud} & 2+1 & 293 & \parbox[t]{4.7cm}{ Chiral fit with a term linear in $M_\pi^2$. } \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
$\chi$QCD 15 & \cite{Gong:2015iir} & 2+1 & 330 & \parbox[t]{4.7cm}{ Chiral fit with a term linear in $M_{\pi^2, {\rm val}}$. }   \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
Engelhardt 12 & \cite{Engelhardt:2012gd} & 2+1 & 495, 356, 293 & \parbox[t]{4.7cm}{Value from chiral log fit. Difference from constant fit added as a 
 systematic uncertainty.}   \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
ETM 17C & \cite{Alexandrou:2017oeh} & 2 & 130 & \parbox[t]{4.7cm}{Single simulation at $M_\pi = 130$ MeV. }  \\[0.5ex]\\[0.5ex]
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hline\hline
\end{tabular*}
\caption{
\ifx\reducedapptables\undefined
Chiral extrapolation/minimum pion mass in determinations of $g_A^q$.
\else
Chiral extrapolation/minimum pion mass in determinations of $g_A^q$ and $g_T^q$.
\fi
}
}
\end{table}


\begin{table}[!ht]
{\footnotesize
\begin{tabular*}{\textwidth}{l @{\extracolsep{\fill}} c c c c l}
\hline\hline \\[-1.0ex]
Collab. & Ref. & $\Nf$ & $L$ [fm] & ${M_{\pi,\rm min}}L$ & Description 
\\[.3ex]\\[-2.ex] \hline \hline \\[-1.0ex]
%
%%% SS
ETM 19 & \cite{Alexandrou:2019brg} & 2+1+1 & \parbox[t]{1.4cm}{5.1} &
\parbox[t]{1.cm}{3.6} & \parbox[t]{6.3cm}{FVE are anticipated to be small based on an investigation using two
near physical point $\Nf=2$ ensembles with $M_\pi L=3.0$ and $4.0$.}
\\[0.5ex]\\[0.5ex]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifx\reducedapptables\undefined
\hline \\[-0.5ex]
PNDME 18A & \cite{Lin:2018obj} & 2+1+1 & \parbox[t]{1.4cm}{2.4,\\2.9--3.8,\\2.8--5.6,\\2.8} & \parbox[t]{1.cm}{3.9,\\4.4,\\3.9,\\4.5} & \parbox[t]{4.7cm}{ Connected: Joint continuum, chiral and volume fit with the term  $M_\pi^2 e^{-M_\pi L}$. \\ Disconnected: Neglect volume dependence. }  \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
$\chi$QCD 18 & \cite{Liang:2018pis} & 2+1 & \parbox[t]{1.4cm}{4.6,\\2.7,\\2.6} & \parbox[t]{1.cm}{4.0,\\4.5,\\4.1} &  \parbox[t]{4.7cm}{ FV correction expected to be small. }\\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
JLQCD 18 & \cite{Yamanaka:2018uud} & 2+1 & \parbox[t]{1.4cm}{1.8--2.7} & \parbox[t]{1.cm}{4.0} & \parbox[t]{4.7cm}{ FV correction expected to be small. }  \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
$\chi$QCD 15 & \cite{Gong:2015iir} & 2+1 & \parbox[t]{1.4cm}{2.6} & \parbox[t]{1.cm}{3.3} &  \parbox[t]{4.7cm}{ FV correction neglected. }   \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
Engelhardt 12 & \cite{Engelhardt:2012gd} & 2+1 & \parbox[t]{1.4cm}{2.5} & \parbox[t]{1.cm}{3.7} & \parbox[t]{4.7cm}{ A generic 10\% error is added based on possible FVE in $g_A$.}   \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
ETM 17C & \cite{Alexandrou:2017oeh} & 2 & \parbox[t]{1.4cm}{3.7} & \parbox[t]{1.cm}{3.0} &  \parbox[t]{5.2cm}{Single simulation with $M_\pi L = 3.0$. }  \\[0.5ex]\\[0.5ex]
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hline\hline
\end{tabular*}
\caption{
\ifx\reducedapptables\undefined
Finite-volume effects in determinations of $g_A^q$.
\else
Finite-volume effects in determinations of $g_A^q$ and $g_T^q$.
\fi
}
}
\end{table}


\begin{table}[!ht]
{\footnotesize
\begin{tabular*}{\textwidth}{l @{\extracolsep{\fill}} c c c }
\hline\hline \\[-1.0ex]
Collab. & Ref. & $\Nf$ & Ren. 
\\[.3ex]\\[-2.ex] \hline \hline \\[-1.0ex]
%
%%% SS
ETM 19 & \cite{Alexandrou:2019brg} & 2+1+1 & RI-SMOM   \\[0.5ex]\\[0.5ex]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifx\reducedapptables\undefined
\hline \\[-0.5ex]
PNDME 18A & \cite{Lin:2018obj} & 2+1+1 & RI-SMOM    \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
$\chi$QCD 18 & \cite{Liang:2018pis} & 2+1 & NP    \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
JLQCD 18 & \cite{Yamanaka:2018uud} & 2+1 & RI-MOM    \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
$\chi$QCD 15 & \cite{Gong:2015iir} & 2+1 & NP    \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
Engelhardt 12 & \cite{Engelhardt:2012gd} & 2+1 & NP    \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
ETM 17C & \cite{Alexandrou:2017oeh} & 2 & RI'-MOM    \\[0.5ex]\\[0.5ex]
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \hline \hline \\[-1.0ex]
\end{tabular*}
\caption{
\ifx\reducedapptables\undefined
Renormalization in determinations of $g_A^q$.
\else
Renormalization in determinations of $g_A^q$ and $g_T^q$.
\fi
}
}
\end{table}
\begin{table}[!ht]

{\footnotesize
\begin{tabular*}{\textwidth}{l @{\extracolsep{\fill}} c c c l}
\hline\hline \\[-1.0ex]
Collab. & Ref. & $\Nf$ & $\tau$ [fm] & Description 
\\[.3ex]\\[-2.ex]\hline \hline \\[-1.0ex]
%
%%% SS
ETM 19 & \cite{Alexandrou:2019brg} & 2+1+1 &  \parbox[t]{3.5cm}{[0.6--1.6]/all}  &  \parbox[t]{6.3cm}{Two-state fit to all $\tau$. A comparison is made with three-state fits, plateau fits and the summation method.} \\[0.5ex]\\[0.5ex]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifx\reducedapptables\undefined
\hline \\[-0.5ex]
PNDME 18A & \cite{Lin:2018obj} & 2+1+1 & \parbox[t]{3.5cm}{[0.8--1.4]\par [1.0--1.4,0.9--1.4]\par [0.9--1.2,0.9--1.2,0.7--1.4]\par [0.9--1.4]} &  \parbox[t]{4.7cm}{ Connected: three-state fit. \\ Disconnected: two-state fit.} \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
$\chi$QCD 18 & \cite{Liang:2018pis} & 2+1 & \parbox[t]{3.5cm}{[1.0--1.6]\par [0.9--1.3]\par [1.0--1.2]} & \parbox[t]{4.7cm}{ Two-state fit. }  \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
JLQCD 18 & \cite{Yamanaka:2018uud} & 2+1 & \parbox[t]{3.5cm}{[1.0--1.54]} &   \parbox[t]{4.7cm}{ Constant fit to all $\tau$ \\ and $t \in [4 - (\tau-4)] $ data. } \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
$\chi$QCD 15 & \cite{Gong:2015iir} & 2+1 & \parbox[t]{3.5cm}{[0.68--1.14]} & \parbox[t]{4.7cm}{ Two-state fit. }  \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
Engelhardt 12 & \cite{Engelhardt:2012gd} & 2+1 & \parbox[t]{3.5cm}{[1.24--1.5]} & \parbox[t]{4.7cm}{Not quantified.}  \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
ETM 17C & \cite{Alexandrou:2017oeh} & 2 & \parbox[t]{3.5cm}{[0.9--1.3]} & \parbox[t]{4.7cm}{ Plateau value at 1.31 fm. Included systematic error as the difference from the two-state fit.} \\[0.5ex]\\[0.5ex]
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hline \hline \\[-1.0ex]
\end{tabular*}
\caption{
\ifx\reducedapptables\undefined
Control of excited state contamination in determinations of $g_A^q$.
\else
Control of excited state contamination in determinations of $g_A^q$ and $g_T^q$.
\fi
The comma-separated list of numbers in square brackets denote the range of source-sink separations $\tau$ (in fermi) at each value of the bare coupling. } }
\end{table}


==> NME/Tables/app_gt_singlet.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifx\reducedapptables\undefined
\begin{table}[!ht]

{\footnotesize
\begin{tabular*}{\textwidth}{l @{\extracolsep{\fill}} c c c l}
\hline\hline \\[-1.0ex]
Collab. & Ref. & $\Nf$ & $a$ [fm] & Description 
\\[.3ex]\\[-2.ex] \hline \hline \\[-1.0ex]
%
%%% SS
ETM 19 & \cite{Alexandrou:2019brg} & 2+1+1 & 0.08 & \parbox[t]{6.3cm}{Not estimated. }
\\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
PNDME 18B & \cite{Gupta:2018lvp} & 2+1+1 & 0.15,0.12,0.09,0.06 & \parbox[t]{4.7cm}{  Connected: Joint continuum, chiral and volume fit with a term linear in $a$. \\ Disconnected: Joint continuum and chiral fit with a term linear in $a$. } \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
PNDME 16 & \cite{Bhattacharya:2016zcn} & 2+1+1 & 0.12,0.09,0.06 &\parbox[t]{4.7cm}{  Connected: Joint continuum, chiral and volume fit with a term linear in $a$. \\ Disconnected contribution neglected. } \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
PNDME 15 & \cite{Bhattacharya:2015wna,Bhattacharya:2015esa} & 2+1+1 & 0.12,0.09,0.06 &  \parbox[t]{4.7cm}{ Connected: Joint continuum, chiral and volume fit with a term linear in $a$. \\ Disconnected strange: Joint continuum and chiral fit with a term linear in $a$. } \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
JLQCD 18 & \cite{Yamanaka:2018uud} & 2+1 & 0.11 &   \parbox[t]{4.7cm}{  Discretization effects are estimated to be $8\%$ using $\cO(\Lambda^2_{QCD}a^2)$ with $\Lambda_{QCD}\approx 500$~MeV.} \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
ETM 17 & \cite{Alexandrou:2017qyt} & 2 & 0.09 &  \parbox[t]{4.7cm}{ Single lattice spacing.}  \\[0.5ex]\\[0.5ex]
\hline \hline \\[-1.0ex]
\end{tabular*}
\caption{Continuum extrapolations/estimation of lattice artifacts in determinations of $g_T^q$.}
}
\end{table}

\begin{table}[!ht]
{\footnotesize
\begin{tabular*}{\textwidth}{l @{\extracolsep{\fill}} c c c l}
\hline\hline \\[-1.0ex]
{Collab.} & {Ref.} & {$\Nf$} & {$M_{\pi,\rm min}\,[\mev]$} & {Description}  
\\[.3ex]\\[-2.ex] \hline \hline \\[-1.0ex]
%
%%% SS 
ETM 19 & \cite{Alexandrou:2019brg} & 2+1+1 & 139  & \parbox[t]{6.3cm}{ Simulate close to $M_\pi^{phys}$. }
\\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
PNDME 18B & \cite{Gupta:2018lvp} & 2+1+1 &  \parbox[t]{2.5cm}{ $C$: 320,225,135 \\ $D_l$: 320, 235 \\ $D_s$: 320, 225, 138}&  \parbox[t]{4.7cm}{  Connected: Joint continuum, chiral and volume fit with a term linear in $M_\pi^2$. \par Disconnected: Joint continuum and chiral fit with a term linear in $M_\pi^2$. }  \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
PNDME 16 & \cite{Bhattacharya:2016zcn} & 2+1+1 & \parbox[t]{2.5cm}{ $C$: 310,225,138 } &   \parbox[t]{4.7cm}{  Connected: Joint continuum, chiral and volume fit with a term linear in $M_\pi^2$. } \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
PNDME 15 & \cite{Bhattacharya:2015wna,Bhattacharya:2015esa} & 2+1+1 & \parbox[t]{2.5cm}{ $C$: 310,225,138 \\ $D_s$: 310, 228} & \parbox[t]{4.7cm}{  Connected: Joint continuum, chiral and volume fit with a term linear in $M_\pi^2$. \par Disconnected: Joint continuum and chiral fit with a term linear in $M_\pi^2$. }  \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
JLQCD 18 & \cite{Yamanaka:2018uud} & 2+1 & 293 &  Fit linear in $M_\pi^2$. \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
ETM 17 & \cite{Alexandrou:2017qyt} & 2 & 130 & \parbox[t]{4.7cm}{Single simulation at $M_\pi = 130$ MeV. } \\[0.5ex]\\[0.5ex]
\hline\hline
\end{tabular*}
\caption{Chiral extrapolation/minimum pion mass in determinations of $g_T^q$.}
}
\end{table}

\begin{table}[!ht]
{\footnotesize
\begin{tabular*}{\textwidth}{l @{\extracolsep{\fill}} c c c c l}
\hline\hline \\[-1.0ex]
Collab. & Ref. & $\Nf$ & $L$ [fm] & ${M_{\pi,\rm min}}L$ & Description 
\\[.3ex]\\[-2.ex] \hline \hline \\[-1.0ex]
%
%%% SS
ETM 19 & \cite{Alexandrou:2019brg} & 2+1+1 & \parbox[t]{1.4cm}{5.1} &
\parbox[t]{1.cm}{3.6} & \parbox[t]{6.3cm}{FVE are anticipated to be small based on an investigation using two
near physical point $\Nf=2$ ensembles with $M_\pi L=3.0$ and $4.0$.}
\\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
PNDME 18B & \cite{Gupta:2018lvp} & 2+1+1 & \parbox[t]{1.4cm}{2.4,\\2.9--3.8,\\2.8--5.6,\\2.8} & \parbox[t]{1.cm}{3.9,\\4.4,\\3.9,\\4.5} &  \parbox[t]{4.7cm}{ Connected: Joint continuum, chiral and volume fit with the term  $M_\pi^2 e^{-M_\pi L}$. \\ Disconnected: Neglect volume dependence. }  \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
PNDME 16 & \cite{Bhattacharya:2016zcn} & 2+1+1 & \parbox[t]{1.4cm}{2.9--4.8,\\2.8--5.6,\\2.8--3.7} & \parbox[t]{1.cm}{5.5,\\3.9,\\4.4} & \parbox[t]{4.7cm}{ Connected: Joint continuum, chiral and volume fit with the term  $M_\pi^2 e^{-M_\pi L}$.  }   \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
PNDME 15 & \cite{Bhattacharya:2015wna,Bhattacharya:2015esa} & 2+1+1 & \parbox[t]{1.4cm}{2.9--4.8,\\2.8--5.6,\\2.8--3.7} & \parbox[t]{1.cm}{5.5,\\3.9,\\4.4} & \parbox[t]{4.7cm}{ Connected: Joint continuum, chiral and volume fit with the term  $M_\pi^2 e^{-M_\pi L}$. \\ Disconnected strange: Neglect volume dependence. }   \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
JLQCD 18 & \cite{Yamanaka:2018uud} & 2+1 & \parbox[t]{1.4cm}{1.8--2.7} & \parbox[t]{1.cm}{4.0} &  \parbox[t]{4.7cm}{FV correction expected to be small for $M_\pi L \gtrsim 4$.} \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
ETM 17 & \cite{Alexandrou:2017qyt} & 2 & \parbox[t]{1.4cm}{4.5} & \parbox[t]{1.cm}{3.0} & \parbox[t]{4.7cm}{Single simulation with $M_\pi L = 3.0$. }  \\[0.5ex]\\[0.5ex]
\hline\hline
\end{tabular*}
\caption{Finite-volume effects in determinations of $g_T^q$.}
}
\end{table}


\begin{table}[!ht]
{\footnotesize
\begin{tabular*}{\textwidth}{l @{\extracolsep{\fill}} c c c }
\hline\hline \\[-1.0ex]
Collab. & Ref. & $\Nf$ & Ren. 
\\[.3ex]\\[-2.ex] \hline \hline \\[-1.0ex]
%
%%% SS
ETM 19 & \cite{Alexandrou:2019brg} & 2+1+1 & RI-SMOM   \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
PNDME 18B & \cite{Gupta:2018lvp} & 2+1+1 & RI-SMOM    \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
PNDME 16 & \cite{Bhattacharya:2016zcn} & 2+1+1 & RI-SMOM    \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
PNDME 15 & \cite{Bhattacharya:2015wna,Bhattacharya:2015esa} & 2+1+1 & RI-SMOM    \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
JLQCD 18 & \cite{Yamanaka:2018uud} & 2+1 & NP    \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
ETM 17 & \cite{Alexandrou:2017qyt} & 2 & RI'-MOM    \\[0.5ex]\\[0.5ex]
 \hline \hline \\[-1.0ex]
\end{tabular*}
\caption{Renormalization in determinations of $g_T^q$.}
}
\end{table}
\begin{table}[!ht]

{\footnotesize
\begin{tabular*}{\textwidth}{l @{\extracolsep{\fill}} c c c l}
\hline\hline \\[-1.0ex]
Collab. & Ref. & $\Nf$ & $\tau$ [fm] & Description 
\\[.3ex]\\[-2.ex]\hline \hline \\[-1.0ex]
%
%%% SS
ETM 19 & \cite{Alexandrou:2019brg} & 2+1+1 &  \parbox[t]{3.5cm}{[0.6--1.6]/all}  &  \parbox[t]{6.3cm}{Two-state fit to all $\tau$. A comparison is made with three-state fits, plateau fits and the summation method.} \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
PNDME 18B & \cite{Gupta:2018lvp} & 2+1+1 & \parbox[t]{3.5cm}{[0.8--1.4]\par [1.0--1.4,0.9--1.4]\par [0.9--1.2,0.9--1.2,0.7--1.4]\par [0.9--1.4]} &  \parbox[t]{4.7cm}{ Connected: three-state fit. \\ Disconnected: constant fit.} \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
PNDME 16 & \cite{Bhattacharya:2016zcn} & 2+1+1 & \parbox[t]{3.5cm}{[1.0--1.4,1.0--1.4]\par [0.9--1.2,0.9--1.2,0.9--1.2]\par [0.9--1.4,0.9--1.4]} & \parbox[t]{4.7cm}{ Connected: two-state fit. } \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
PNDME 15 & \cite{Bhattacharya:2015wna,Bhattacharya:2015esa} & 2+1+1 & \parbox[t]{3.5cm}{[1.0--1.4,1.0--1.4]\par [0.9--1.2,0.9--1.2,0.9--1.2]\par [0.9--1.4,0.9--1.4]} & \parbox[t]{4.7cm}{ Connected: two-state fit. \\ Disconnected: two-state fit. } \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
JLQCD 18 & \cite{Yamanaka:2018uud} & 2+1 & \parbox[t]{3.5cm}{[1.0--1.54]} & Constant fit to all data \\[0.5ex]\\[0.5ex]
\hline\\[-0.5ex]
ETM 17 & \cite{Alexandrou:2017qyt} & 2 & \parbox[t]{3.5cm}{[0.9--1.3]} & \parbox[t]{4.5cm}{ $C$:  Plateau fit to 1.31 fm data \\ $D$: Plateau fit to 0.75 fm data}   \\[0.5ex]\\[0.5ex]
\hline \hline \\[-1.0ex]
\end{tabular*}
\caption{Control of excited state contamination in determinations of $g_T^q$. The comma-separated list of numbers in square brackets denote the range of source-sink separations $\tau$ (in fermi) at each value of the bare coupling. } }
\end{table}

\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> Tables/Summarytable5.tex <==
$ \Sigma^{1/3}$[MeV]&\ref{sec:SU2_averages}&$286(23)$&\cite{Cichy:2013gja,Alexandrou:2017bzk}&$272(5)$&\cite{Bazavov:2010yq,Borsanyi:2012zv,Durr:2013goa,Boyle:2015exm,Cossu:2016eqs,Aoki:2017paw}&$266(10)$&\cite{Baron:2009wt,Cichy:2013gja,Brandt:2013dua,Engel:2014eea}\\[1mm]
$ {\Fpi}/{F}$&\ref{sec:SU2_averages}&$1.077(3)$&\cite{Baron:2011sf}&$1.062(7)$&\cite{Bazavov:2010hj,Beane:2011zm,Borsanyi:2012zv,Durr:2013goa,Boyle:2015exm}&$1.073(15)$&\cite{Frezzotti:2008dr,Baron:2009wt,Brandt:2013dua,Engel:2014eea}\\[1mm]
$ \lbar_3$&\ref{sec:SU2_averages}&$3.53(26)$&\cite{Baron:2011sf}&$3.07(64)$&\cite{Bazavov:2010hj,Beane:2011zm,Borsanyi:2012zv,Durr:2013goa,Boyle:2015exm}&$3.41(82)$&\cite{Frezzotti:2008dr,Baron:2009wt,Brandt:2013dua}\\[1mm]
$ \lbar_4$&\ref{sec:SU2_averages}&$4.73(10)$&\cite{Baron:2011sf}&$4.02(45)$&\cite{Bazavov:2010hj,Beane:2011zm,Borsanyi:2012zv,Durr:2013goa,Boyle:2015exm}&$4.40(28)$&\cite{Frezzotti:2008dr,Baron:2009wt,Brandt:2013dua,Gulpers:2015bba}\\[1mm]
$ \lbar_6$&\ref{sec:SU2_averages}&&&&&$15.1(1.2)$&\cite{Frezzotti:2008dr,Brandt:2013dua}\\[1mm]
$ a_0^2\Mpi$&\ref{sec:SU2_averages}&$-0.0441(4)$&\cite{Helmes:2015gla}&&&$-0.04385(47)$&\cite{Feng:2009ij}\\[1mm]
$ \Sigma_0^{1/3}      $[MeV]&\ref{sec:SU3_averages}&&&$245(8)$&\cite{Bazavov:2009fk}&&\\[1mm]
$ \Sigma/\Sigma_0     $&\ref{sec:SU3_averages}&&&$1.48(16)$&\cite{Bazavov:2009fk}&&\\[1mm]
$ F_0                 $[MeV]&\ref{sec:SU3_averages}&&&$80.3(6.0)$&\cite{Bazavov:2010hj}&&\\[1mm]
$ F/F_0               $&\ref{sec:SU3_averages}&&&$1.104(41)$&\cite{Bazavov:2009fk}&&\\[1mm]
$ B/B_0               $&\ref{sec:SU3_averages}&&&$1.21(7)$&\cite{Bazavov:2009fk}&&\\[1mm]
$ L_4 $&\ref{sec:SU3_averages}&$+0.09(34)\times10^{-3}$&\cite{Dowdall:2013rya}&$-0.02(56)\times10^{-3}$&\cite{Bazavov:2010hj}&&\\[1mm]
$ L_5 $&\ref{sec:SU3_averages}&$+1.19(25)\times10^{-3}$&\cite{Dowdall:2013rya}&$+0.95(41)\times10^{-3}$&\cite{Bazavov:2010hj}&&\\[1mm]
$ L_6 $&\ref{sec:SU3_averages}&$+0.16(20)\times10^{-3}$&\cite{Dowdall:2013rya}&$+0.01(34)\times10^{-3}$&\cite{Bazavov:2010hj}&&\\[1mm]
$ L_8 $&\ref{sec:SU3_averages}&$+0.55(15)\times10^{-3}$&\cite{Dowdall:2013rya}&$+0.43(28)\times10^{-3}$&\cite{Bazavov:2010hj}&&\\[1mm]
$ a_0^{1/2}\mu_{\pi K}  $&\ref{sec:SU3_averages}&$0.127(2)$&\cite{Helmes:2018nug}&&&&\\[1mm]
$ a_0^{3/2}\mu_{\pi K}  $&\ref{sec:SU3_averages}&$-0.0463(17)$&\cite{Helmes:2018nug}&&&&\\[1mm]
$ a_0^1 M_K             $&\ref{sec:SU3_averages}&$-0.388(20)$&\cite{Helmes:2017smr}&&&&\\[1mm]
\hline


==> qmass/qmass_mb_app.tex <==
% !TEX root = ../FLAG_master.tex
%\clearpage

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifx\reducedapptables\undefined
\begin{table}[!ht]
{\footnotesize
\begin{tabular*}{\textwidth}[l]{l @{\extracolsep{\fill}} c c c l}
\hline\hline \\[-1.0ex]
Collab. & Ref. & $\Nf$ & $a$ [fm] & Description
\\[1.0ex] \hline \hline \\[-1.0ex]
% 2+1+1
%
HPQCD 21  & \cite{Hatton:2021syc}  & 2+1+1 & \parbox[t]{3cm}{0.03, 0.042, 0.06, 0.09}  & \parbox[t]{4.5cm}{Scale set from $w_0$ and $f_\pi$. HISQ action for charm quarks.} \\
[4.0ex]
\hline\\[-1.0ex]
%
FNAL/MILC/TUMQCD 18  & \cite{Bazavov:2018omf}  & 2+1+1 & \parbox[t]{3cm}{0.03, 0.042, 0.06, 0.09, 0.12, 0.15}  & \parbox[t]{4.5cm}{Scale set from $f_\pi$. HISQ action for charm quarks.} \\
[4.0ex] \hline \\[-1.0ex]
%
Gambino 17 & \cite{Gambino:2017vkx} & 2+1+1 & 0.062, 0.082, 0.089  & \parbox[t]{4.5cm}{Scale set from $f_{\pi^+}$} \\
[1.0ex] \hline \\[-1.0ex]
%
ETM 16B & \cite{Bussone:2016iua} & 2+1+1 &  0.0619, 0.0815, 0.0885  & \parbox[t]{4.5cm}{Scale set from $f_{\pi}$} \\
 \hline \\[-1.0ex]
%
HPQCD 14B  & \cite{Colquhoun:2014ica} & 2+1+1 & 0.09, 0.12, 0.15 & \parbox[t]{4.5cm}{Scale set through the $\Upsilon^\prime-\Upsilon$ mass splitting.} \\
[4.0ex] \hline \\[-1.0ex]
%
ETM 14B & \cite{Bussone:2014cha} & 2+1+1 & 0.062, 0.082, 0.089 & \parbox[t]{4.5cm}{Scale set through $F_\pi$.}\\
[1.0ex] \hline \\[-1.0ex]
%
HPQCD 14A  & \cite{Chakraborty:2014aca} & 2+1+1 & 0.06, 0.09, 0.12, 0.15  & \parbox[t]{4.5cm}{Scale set through the Wilson flow parameter $w_0$.} \\
[4.0ex]
 \hline \hline \\[-1.0ex]
%
\end{tabular*}
\caption{Continuum extrapolations/estimation of lattice artifacts in the determinations of $m_b$ with $\Nf=2+1+1$ quark flavours.}
}
\end{table}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifx\reducedapptables\undefined \begin{table}[!ht]
{\footnotesize
\begin{tabular*}{\textwidth}[l]{l @{\extracolsep{\fill}} c c c l}
\hline\hline \\[-1.0ex]
Collab. & Ref. & $\Nf$ & $a$ [fm] & Description
\\[1.0ex] \hline \hline \\[-1.0ex]
%2+1
%
Petreczky 19  & \cite{Petreczky:2019ozv} & 2+1 & 0.025 to 0.11 fm & \parbox[t]{4.5cm}{HISQ action for the charm quark. Scale set from $r_1$ parameter of heavy quark potential and $f_\pi$.\\}
\\[4.0ex]
\\ [1.0ex] \hline
\\[-1.0ex]
%
Maezawa 16  & \cite{Maezawa:2016vgv} & 2+1 & 0.04 to 0.14 fm & \parbox[t]{4.5cm}{HISQ action for the charm quark. Scale set from $r_1$ parameter of heavy quark potential.\\} \\ 
 \hline
\\[-1.0ex]
%
HPQCD 13B  & \cite{Lee:2013mla} & 2+1 & 0.084, 0.12 & \parbox[t]{4.5cm}{Scale set through the static-quark potential parameter $r_1$.} \\
[4.0ex] \hline \\[-1.0ex]
%
HPQCD 10 & \cite{McNeile:2010ji} & 2+1 & \parbox[t]{3cm}{0.044, 0.059, 0.084, 0.12, 0.15} & \parbox[t]{4.5cm}{Scale set through the static-quark potential parameter $r_1$.} \\
[4.0ex]
 \hline \hline \\[-1.0ex]
%
\end{tabular*}
\caption{Continuum extrapolations/estimation of lattice artifacts in the determinations of $m_b$ with $\Nf=2+1$ quark flavours.}
}
\end{table}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\ifx\reducedapptables\undefined
\begin{table}[!ht]
{\footnotesize
\begin{tabular*}{\textwidth}[l]{l @{\extracolsep{\fill}} c c c}
\hline \hline  \\[-1.0ex]
Collab. & Ref. & $\Nf$ & $M_{\pi,\text{min}}$ [MeV] 
\\[1.0ex] \hline \hline \\[-1.0ex]
% 2+1+1
%
HPQCD 21  & \cite{Hatton:2021syc}  & 2+1+1 & physical \\
[1.0ex]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
[4.0ex]\hline\\[-1.0ex]
%
FNAL/MILC/TUMQCD 18  & \cite{Bazavov:2018omf} & 2+1+1 & $130$ ($173_{RMS}$) \\
[1.0ex] \hline \\[-1.0ex]
%
Gambino 17 & \cite{Gambino:2017vkx} & 2+1+1 & $210 $ \\
[1.0ex] \hline \\[-1.0ex]
%
ETM 16B & \cite{Bussone:2016iua} &  2+1+1 & $210 $ \\
 \hline \\[-1.0ex]
%
HPQCD 14B  & \cite{Colquhoun:2014ica} & 2+1+1 & 306,  128 \\
[1.0ex] \hline \\[-1.0ex]
%
ETM 14B & \cite{Bussone:2014cha} & 2+1+1 &  210  \\
[1.0ex] \hline \\[-1.0ex]
% 
HPQCD 14A  & \cite{Chakraborty:2014aca} & 2+1+1 & $128_{\pi, 5}$ ($173_{RMS}$) \\
[1.0ex]
 \hline \hline \\[-1.0ex]
%
\end{tabular*}
\caption{Chiral extrapolation/minimum pion mass in the determinations of $m_b$ with $\Nf=2+1+1$ quark flavours.}
}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifx\reducedapptables\undefined
\begin{table}[!ht]
{\footnotesize
\begin{tabular*}{\textwidth}[l]{l @{\extracolsep{\fill}} c c c}
\hline \hline  \\[-1.0ex]
Collab. & Ref. & $\Nf$ & $M_{\pi,\text{min}}$ [MeV] 
\\[1.0ex] \hline \hline \\[-1.0ex]
%
Petreczky 19  & \cite{Petreczky:2019ozv} & 2+1 & 161 \\ [1.0ex] 
\hline
\\[-1.0ex]
% 2+1
Maezawa 16  & \cite{Maezawa:2016vgv} & 2+1 & 160   \\
[1.0ex]
 \hline \\[-1.0ex]
%
HPQCD 13B  & \cite{Lee:2013mla} & 2+1 & 345  \\
[1.0ex] \hline \\[-1.0ex]
%
HPQCD 10 & \cite{McNeile:2010ji} & 2+1 & 260  \\
[1.0ex]
 \hline \hline \\[-1.0ex]
%
\end{tabular*}
\caption{Chiral extrapolation/minimum pion mass in the determinations of $m_b$ with $\Nf=2+1$ quark flavours.}
}
\end{table}

\newpage
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifx\reducedapptables\undefined
\begin{table}[!ht]
{\footnotesize
\begin{tabular*}{\textwidth}[l]{l @{\extracolsep{\fill}} c c c c}
\hline\hline  \\[-1.0ex]
Collab. & Ref. & $\Nf$ & $L$ [fm] & $M_{\pi,\text{min}} L$ 
\\[1.0ex] \hline \hline \\[-1.0ex]
% 2+1+1
%
HPQCD 21  & \cite{Hatton:2021syc}  & 2+1+1 &  1.9 - 5.76 & 3.8\\
[1.0ex]
[4.0ex]\hline\\[-1.0ex]
%
FNAL/MILC/TUMQCD 18  & \cite{Bazavov:2018omf} & 2+1+1 & 2.89 - 6.12  & 3.7 \\
[1.0ex] \hline \\[-1.0ex]
%
Gambino 17 & \cite{Gambino:2017vkx} & 2+1+1 & $2.7_{\pi^0}$ ($3.3_{\pi^\pm}$) \\
[1.0ex] \hline \\[-1.0ex]
%
ETM 16B & \cite{Bussone:2016iua}  & 2+1+1 & $2.7_{\pi^0}$ ($3.3_{\pi^\pm}$) \\
 \hline \\[-1.0ex]
%
HPQCD 14B  & \cite{Colquhoun:2014ica} & 2+1+1 & 2.4-7.8 & 3.0-3.8 \\
[1.0ex] \hline \\[-1.0ex]
%
ETM 14B & \cite{Bussone:2014cha} & 2+1+1 &  1.9-2.8 & 3.0-5.8   \\
[1.0ex] \hline \\[-1.0ex]
%
HPQCD 14A  & \cite{Chakraborty:2014aca} & 2+1+1 & 2.5-5.8  & 3.7  \\
[1.0ex]
 \hline \hline \\[-1.0ex]
%
\end{tabular*}
\caption{Finite-volume effects in the determinations of $m_b$ with $\Nf=2+1+1$ quark flavours.}
}
\end{table}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifx\reducedapptables\undefined
\begin{table}[!ht]
{\footnotesize
\begin{tabular*}{\textwidth}[l]{l @{\extracolsep{\fill}} c c c c}
\hline\hline  \\[-1.0ex]
Collab. & Ref. & $\Nf$ & $L$ [fm] & $M_{\pi,\text{min}} L$ 
\\[1.0ex] \hline \hline \\[-1.0ex]
% 2+1
%
Petreczky 19  & \cite{Petreczky:2019ozv} & 2+1 &  1.6 -- 5.2 & 4.2 \\ [1.0ex]
 \hline
\\[-1.0ex]
%
Maezawa 16  & \cite{Maezawa:2016vgv} & 2+1 & 2.6 -- 5.2 & 4.2  \\ 
[1.0ex]
 \hline \\[-1.0ex]
%
HPQCD 13B  & \cite{Lee:2013mla} & 2+1 & 2.4, 3.4 & 4.1  \\
[1.0ex] \hline \\[-1.0ex]
%
HPQCD 10 & \cite{McNeile:2010ji} & 2+1 & 2.3 -- 3.4 & 3.8  \\
[1.0ex] 
\hline \hline \\[-1.0ex]
%
\end{tabular*}
\caption{Finite-volume effects in the determinations of $m_b$ with $\Nf=2+1$ quark flavours.}
}
\end{table}
 \fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifx\reducedapptables\undefined

\begin{table}[!ht]
{\footnotesize
\begin{tabular*}{\textwidth}[l]{l @{\extracolsep{\fill}} c c c c}
\hline\hline  \\[-1.0ex]
Collab. & Ref. & $\Nf$ & $L$ [fm] & $M_{\pi,\text{min}} L$ 
\\[1.0ex] \hline \hline \\[-1.0ex]
% 2
ETM 13B & \cite{Carrasco:2013zta} & 2 & $\gtrsim 2.0$ & 3.5   \\
[1.0ex] \hline \\[-1.0ex]
%
ALPHA 13C& \cite{Bernardoni:2013xba} & 2 & 2.3--3.6 & 4.1 \\
[1.0ex] \hline \\[-1.0ex]
%
ETM 11A & \cite{Dimopoulos:2011gx} & 2 & $\gtrsim 2.0$ & 3.5  \\
[1.0ex]
 \hline \hline \\[-1.0ex]
%
\end{tabular*}
\caption{Finite-volume effects in the determinations of $m_b$ with $\Nf=2$ quark flavours.}
}
\end{table}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifx\reducedapptables\undefined
\begin{table}[!ht]
{\footnotesize
\begin{tabular*}{\textwidth}[l]{l @{\extracolsep{\fill}} c c l}
\hline\hline \\[-1.0ex]
Collab. & Ref. & $\Nf$  & Description
\\[1.0ex] \hline \hline \\[-1.0ex]
%
% 2+1+1
%
ETM 21A  & \cite{Alexandrou:2021gqw}  & 2+1+1 &  Nonperturbative (RI/MOM) \\
[2.0ex]
\hline\\[-1.0ex]
%
HPQCD 21 & \cite{Hatton:2021syc}  & 2+1+1 &  Scale dependence enters through QED\\
[4.0ex]\hline\\[-1.0ex]
%
FNAL/MILC/TUMQCD 18 & \cite{Bazavov:2018omf}& 2+1+1 & Renormalization not required. \\
[1.0ex] \hline \\[-1.0ex]
%
Gambino 17 & \cite{Gambino:2017vkx}& 2+1+1 & \parbox[t]{4.5cm}{Nonperturbative renormalization (RI/MOM). }\\
[4.0ex] \hline \\[-1.0ex]
% 
ETM 16B & \cite{Bussone:2016iua} & 2+1+1 & \parbox[t]{4.5cm}{Nonperturbative renormalization (RI/MOM). }\\
[4.0ex]
 \hline \\[-1.0ex]
% 
HPQCD 14B & \cite{Colquhoun:2014ica} & 2+1+1 & \parbox[t]{4.5cm}{Renormalization not required.}\\
[1.0ex] \hline \\[-1.0ex]
%
ETM 14B& \cite{Bussone:2014cha} & 2+1+1 & \parbox[t]{4.5cm}{Nonperturbative renormalization (RI/MOM). }\\
[4.0ex] \hline \\[-1.0ex]
% 
HPQCD 14A & \cite{Chakraborty:2014aca} & 2+1+1 & \parbox[t]{4.5cm}{Renormalization not required. }\\
[1.0ex] 
\hline \hline \\[-1.0ex]
%
\end{tabular*}
\caption{Lattice renormalization in the determinations of $m_b$ with $\Nf=2+1+1$ flavours.}
}
\end{table}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ifx\reducedapptables\undefined
\begin{table}[!ht]
{\footnotesize
\begin{tabular*}{\textwidth}[l]{l @{\extracolsep{\fill}} c c l}
\hline\hline \\[-1.0ex]
Collab. & Ref. & $\Nf$  & Description
\\[1.0ex] \hline \hline \\[-1.0ex]
% 2+1
%
Petreczky 19  & \cite{Petreczky:2019ozv} & 2+1  & not required \\
[2.0ex]
 \hline \\[-1.0ex]
\\[-1.0ex]
%
Maezawa 16  & \cite{Maezawa:2016vgv} & 2+1 & Renormalization not required. \\ [1.0ex] 
\hline
\\[-1.0ex]
%
HPQCD 13B  & \cite{Lee:2013mla} & 2+1 & \parbox[t]{4.5cm}{Renormalization not required.} \\
[1.0ex] \hline \\[-1.0ex]
%
HPQCD 10 & \cite{McNeile:2010ji} & 2+1 &  \parbox[t]{4.5cm}{Renormalization not required.} \\
[1.0ex]
 \hline \hline \\[-1.0ex]
%
\end{tabular*}
\caption{Lattice renormalization in the determinations of $m_b$ with $\Nf=2+1$ flavours.}
}
\end{table}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%









%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "FLAG_master"
%%% End: 

